Summarizing Labeled Multi-Graphs

Real-world graphs can be difficult to interpret and visualize beyond a certain size. To address this issue, graph summarization aims to simplify and shrink a graph, while maintaining its high-level structure and characteristics. Most summarization methods are designed for homogeneous, undirected, simple graphs; however, many real-world graphs are ornate; with characteristics including node labels, directed edges, edge multiplicities, and self-loops. In this paper we propose LM-Gsum, a versatile yet rigorous graph summarization model that (to the best of our knowledge, for the first time) can handle graphs with all the aforementioned characteristics (and any combination thereof). Moreover, our proposed model captures basic sub-structures that are prevalent in real-world graphs, such as cliques, stars, etc. LM-Gsum compactly quantifies the information content of a complex graph using a novel encoding scheme, where it seeks to minimize the total number of bits required to encode (i) the summary graph, as well as (ii) the corrections required for reconstructing the input graph losslessly. To accelerate the summary construction, it creates super-nodes efficiently by merging nodes in groups. Experiments demonstrate that LM-Gsum facilitates the visualization of real-world complex graphs, revealing interpretable structures and high- level relationships. Furthermore, LM-Gsum achieves better trade-off between compression rate and running time, relative to existing methods (only) on comparable settings.

==> symbols.tex <==
Table~\ref{tab:symbols} lists the main symbols used in our notation.

%---------------------------------------------------------------------
% Table of Symbols
%---------------------------------------------------------------------
\begin{table}[htb]
	\caption{Table of symbols.}  
	\label{tab:symbols}
	\centering
	\begin{tabular} {c|l} 
	  \hline
			\textbf{Symbols} & \textbf{Definitions} \\ \hline
			$X$ & A point-cloud dataset within domain $\mathbb{X}$. $X \subseteq \mathbb{X}$ \\
			$n$ & Number of instances in $X$, i.e. cardinality. $n=\left|X\right|$ \\
			$x_i$ & An instance from $X$. $x_i \in X$ \\
			$d$ & Distance function $d : \mathbb{X} \times \mathbb{X} \xrightarrow{} \mathbb {R}$. \\
			$d(x_i, x_j)$ & Distance between instances $x_i, x_j \in X$. \\
			$T$ & A Slim-tree created from $X$. \\
            $s$ & Size of $T$, i.e. total number of nodes. \\
            %$N$ & number of objects \\
            $h$ & Height of $T$, i.e. length of the longest path from the root. \\
            $l$ & Current tree level, i.e. the level of $T$ that is under \\ 
                & consideration at a given moment. $0 \leq l \leq h$ \\
            $c$ & Maximum node capacity for $T$. \reminder{leaf or index nodes?} \\
            %$Ni$ & maximum number of objects in index nodes \\
            $x_{cur}$ & Current instance, i.e. the one under consideration at \\
                      & a given moment. $x_{cur} \in X$\\
            $x_{rep}$ & Representative of the leaf node that stores $x_{cur}$ in $T$. \\
                      & $x_{rep} \in X$ \\
            $x_{crep}$ & Representative of the leaf node that is the closest to $x_{cur}$ in $T$. \\
                      & $x_{crep} \in X$ \\
            $x_{root}$ & Instance in the root node of $T$ that is the closest to $x_{cur}$. \\ 
                       & $x_{root} \in X$ \\
            $x_{1NN}$ & Instance in $T$ that is, approximately, the closest to $x_{cur}$. \\ 
                       & $x_{1NN} \in X$ \\
            $d_{rep}$ & Shortcut for $d(x_{cur}, x_{rep})$. \\
            $d_{root}$ & Shortcut for $d(x_{cur}, x_{root})$. \\
            $d_{crep}$ & Shortcut for $d(x_{cur}, x_{crep})$. \\
            $d_{1NN}$ & Shortcut for $d(x_{cur}, x_{1NN})$. \\
		\hline
	\end{tabular}
\end{table}
%---------------------------------------------------------------------
